DeepHunter: A Graph Neural Network Based Approach for Robust Cyber Threat Hunting

Cyber Threat hunting is a proactive search for known attack behaviors in the organizational information system. It is an important component to mitigate advanced persistent threats (APTs). However, the attack behaviors recorded in provenance data may not be completely consistent with the known attack behaviors. In this paper, we propose DeepHunter, a graph neural network (GNN) based graph pattern matching approach that can match provenance data against known attack behaviors in a robust way. Specifically, we design a graph neural network architecture with two novel networks: attribute embedding networks that could incorporate Indicators of Compromise (IOCs) information, and graph embedding networks that could capture the relationships between IOCs. To evaluate DeepHunter, we choose five real and synthetic APT attack scenarios. Results show that DeepHunter can hunt all attack behaviors, and the accuracy and robustness of DeepHunter outperform the state-of-the-art method, Poirot.

==> discussion.tex <==
%\section{DISCUSSION $\&$ LIMITATIONS}\label{discussion}
\section{DISCUSSION}\label{discussion}
%\subsection{Adversarial Attacks}
In this section, we discuss the evasion attacks on our proposed GNN-based model. Similar to other vulnerable GNN-based models (e.g., node classification~\cite{zugner2018adversarial}, link prediction~\cite{rahwan2019attacking}), recent literature~\cite{zhang2020adversarial} shows that the deep graph matching model is also sensitive to adversarial attacks, i.e., carefully designed small perturbations in graph structures and node attributes. 
However, generating attack samples is difficult in our setting due to two reasons. 

First, to compromise the graph matching model, the attacker should add perturbations on both the query graph and the provenance graph. However, the query graph is usually constructed by analysts or reviewed manually. Moreover, the query graph is usually small. So the perturbations in the query graph can be easily detected by analysts.

Second, it is challenging for an attacker to change the provenance graph (i.e., the system entity's attributes and the topological relations) under an environment where the provenance system is running. Certainly, the attacker can directly tamper with the audit logs~\cite{incidentResponseReport,destroyinglogs} of provenance systems to obtain a suitable compromise. But solving the detection of tampering in audit logs is out of the scope of our research. We refer the reader to the paper~\cite{paccagnella2020custos}. 




%Experiments in Section~\ref{eva:robustness} demonstrate that DeepHunter can tolerate a certain degree of inconsistency. As mentioned in Section~\ref{introduction}, the inconsistencies that our work focuses on are caused by \textcircled{1} the provenance system; and \textcircled{2} attack mutations. However, the attack scenarios for evaluations do not involve adversarial attacks (e.g. , the poisoning attacks and evasion attacks) on the proposed GNN-based graph match model. Adversaries may steer attack behaviors to cause perturbations (node attributes or graph structure) of a provenance graph, which can fool the graph match model. But conducting this attack is challenging because provenance graphs contain complex structural information that is difficult to modify without affecting the attack. Alternatively, adversaries can directly tamper the audit logs~\cite{incidentResponseReport,destroyinglogs} of provenance systems. Solving the detection of tampering in audit logs is outside the scope of our research. We refer the reader to ~\cite{paccagnella2020custos} for more details. 

%Recently, although an increasing number of works start to study the adversarial attacks on deep neural networks, the related study on graph data is at its infancy. The basic idea of many adversarial attack methods is to perturb graph structures and node attributes so that the graph neural networks cannot correctly classify certain nodes or achieve overall performance. Fortunately, as far as we know, there is no new adversarial attacks against the architecture of our proposed graph match network (i.e. graph metric learning architecture).  



%\subsection{The Locating Algorithm}
%We explained the Algorithm~\ref{alg:Framwork} of preprocessing provenance graphs in  Section~\ref{eva:preprocessProvenance}. Specifically, we do not search the entire provenance graph, but only subgraphs based on out-of-band threat intelligence, for suspicious behaviors (query graphs). We believe that this concession is reasonable and matches real analyst workflows fairly accurately. Moreover, DeepHunter can be used to inspect the results of Poirot, which can improve the performance of Poirot.



